Knowledge-rich Image Gist Understanding Beyond Literal Meaning

We investigate the problem of understanding the message (gist) conveyed by images and their captions as found, for instance, on websites or news articles. To this end, we propose a methodology to capture the meaning of image-caption pairs on the basis of large amounts of machine-readable knowledge that has previously been shown to be highly effective for text understanding. Our method identifies the connotation of objects beyond their denotation: where most approaches to image understanding focus on the denotation of objects, i.e., their literal meaning, our work addresses the identification of connotations, i.e., iconic meanings of objects, to understand the message of images. We view image understanding as the task of representing an image-caption pair on the basis of a wide-coverage vocabulary of concepts such as the one provided by Wikipedia, and cast gist detection as a concept-ranking problem with image-caption pairs as queries. To enable a thorough investigation of the problem of gist understanding, we produce a gold standard of over 300 image-caption pairs and over 8,000 gist annotations covering a wide variety of topics at different levels of abstraction. We use this dataset to experimentally benchmark the contribution of signals from heterogeneous sources, namely image and text. The best result with a Mean Average Precision (MAP) of 0.69 indicate that by combining both dimensions we are able to better understand the meaning of our image-caption pairs than when using language or vision information alone. We test the robustness of our gist detection approach when receiving automatically generated input, i.e., using automatically generated image tags or generated captions, and prove the feasibility of an end-to-end automated process.

==> preliminaries.tex <==
\section{Preliminaries}\label{prelim}

%\simpletodo{Replace entity, vertex, concept with "node".}

%\simpletodo {too much focus on the graph}
\noindent The main idea behind our approach is that a general-purpose knowledge
base such as Wikipedia can aid the algorithmic understanding of the message
conveyed by image and caption. 
We hypothesize that the way articles and categories are connected in Wikipedia can be exploited to identify nodes that capture the gist of the image-caption pair.  
%Therefore, in this paper, we place a particular focus on the \emph{ graph structure} of the knowledge base. 


\subsection{Knowledge Graphs}
\noindent Given a knowledge base, we define a \textbf{knowledge graph} as the directed or undirected graph $\mathbf{KG}(V,E, T, \tau)$ such that the set of nodes $V$ contains all nodes representing entities in the knowledge base, every edge $e_{ij} \in E$ corresponds to one relation in the knowledge base between two nodes $v_i$ and $v_j$, the set $T$ contains the relation types in the knowledge base, and the function $\tau:E\rightarrow T$ assigns each edge in $E$ exactly one type in $T$.
In this paper, we mostly consider the knowledge graph undirected, unless specified otherwise. 
In the following, we shortly explain preliminaries that are applied within our pipeline, but that are not part of our contribution.
%duplicate with relatedness paragraph
%To refer to a particular edge (relation) in the knowledge graph, we use the notation $s\stackrel{r}{\rightarrow}t$, which identifies the relation of type $r$ that starts at node $s$ and points to node $t$. 

%A \emph{subgraph} of the knowledge graph $\mathbf{KG}$ is a graph whose set of nodes is a subset of $V$, its set of edges is a subset of $E$, and the set of edge types is a subset of $T$.
%A \emph{path} through the knowledge graph represents a sequence of edges such that every two consecutive edges are connected through a common node, and every node can occur only once. 
%The \emph{path length} is the number of edges on a path. 
%The \emph {shortest path} between two nodes is the path connecting them that traverses the smallest number of edges. 
 %

 
%Consequently, our hunch is that both the caption
%and the image will contain cues about the gist (i.e., message) of the figure. Within this work, we represent a gist as a set of entities and categories in the Wikipedia knowledge base that represent this message best.
%\medskip
%After linking concepts from caption and
%image to the knowledge base, our approach leverages the graph structure
%within the knowledge base and a graph labeling approach to reason about which entities and categories
%capture the message of the image-caption pair.
 

\medskip \noindent \textbf{Node properties.}
One of the most commonly used properties of nodes is their \emph{degree}~\cite{Griffiths07topicsin}.
The degree of a node is the count of all edges that are adjacent to it. Another property of nodes is their tendency of being part of triangles called \emph{local clustering coefficient}~\cite{Griffiths07topicsin}. 
It is computed as the probability that any two random neighbors of a node are connected themselves.  
% whereas a directed graph distinguishes \emph{in-degree} and \emph{out-degree}, which counts the edges either pointing to the node or away from it. 
%
%In directed graphs, the distinction is made between the \emph{in-degree} and \emph{out-degree} of a node. 
%The first counts the number of edges that point to the node of interest, while the second counts the edges that point away from it. 
%For undirected graphs, the degree of a vertex is simply the count of all edges that are adjacent to it. 
%In a knowledge graph, entities that have high degree are entities that are directly linked to many other entities. 
%
%For instance, the category node \emph{Eukaryote}, its connected nodes are less likely to be pairwise inter-connected themselves, then in the category node \emph{Primates}.
%The intuition for knowledge graphs is that nodes with a high clustering coefficient are more specific than those with low clustering coefficient.
Our intuition is that these measures help to find a balance between specific and trivial nodes, and thus, the correct gist nodes. 
%a gist node with a high degree or low clustering coefficient might be too trivial while a gist node with a small degree might be too specific.
The degree and clustering coefficient of nodes are local measures that describe the nodes only in their closest vicinity. 
%The next class of graph measures, assess more complex properties of nodes based on their connectivity to all the other nodes in the graph. 


\medskip \noindent \textbf{Graph centrality measures.}
In the domain of network analysis, a wide range of graph centrality measures have been used with the purpose of locating the most important or influential nodes in the network. 
%One of the most prominent such measures from link analysis is PageRank~\cite{PageRank}. 
%and HITS~\cite{kleinberg1999authoritative}. 
The PageRank~\cite{BrinPage:98} scores nodes based on their stationary probability that a random surfer will visit them.
%HITS~\cite{kleinberg1999authoritative} defines two mutually recursive scores: an authority score, which accounts for how many and how important the hubs who link to the node  are, and a hub score: which accounts for how many and how important the authorities it links to are. 
%We further consider a measure from social network analysis~\cite{Freeman78centralityin}:
Betweeness centrality~\cite{Freeman78centralityin} defines a node as the more important the more often it lies on the shortest path between any two nodes in the graph. 

%As we later detail, we use node centrality measures as features for gist candidates, under the intuition that good gist nodes are central with respect to objects in images and entity mentions in captions. 

Given a knowledge graph $\mathbf{KG}$, as we detail later, our approach makes use of a distance metric $\sigma^{(-1)}: V\times V  \rightarrow \mathbb{R}^+$ between two nodes. This metric captures the inverse of a similarity, relatedness, or semantic association measure between the concepts that are represented by the nodes.
In principle there are two classes of measures, these are (i) those based on textual content associated with nodes, and (ii) those based on the structure of the graph. 
In this work, we use both content- and graph-connectivity measures. 


\subsection{Concept Relatedness}

\medskip \noindent \textbf{Content-based relatedness.} 
Additionally to the previously described graph-connectivity measure, we incorporate a content-based measure of relatedness. 
As each node in the DBpedia knowledge graph has a corresponding article in Wikipedia, we leverage a retrieval index on Wikipedia articles.
For a given concept mention, an object tag, or textual representation of the whole image-caption pair, we can use a retrieval model, which uses a query likelihood, to associate a measure of relevance with each node.

%In this work, we use the sequential dependence model \cite{metzler2005sdm}, which combines the query likelihood model on unigrams, with sequential bigrams and skip-grams up to eight terms distance.

%\simpletodo{We then point here from Step 1, where we use retrieval of individual mentinos and tags; Then we point here from Step 5, where we use the textual representation of the whole-image caption pair.  -> Todo for Laura}


\medskip \noindent \textbf{Graph-based relatedness.} 
A great variety of semantic relatedness measures have been studied~\cite{ZhangGC13}.
%Two of the main classes of measures are (i) those computed based on statistics over an unstructured corpus of documents, and (ii) those that use an external (semi-)structured knowledge base like Wikipedia. 
%In this work, we are particularly interested in the second class of approaches, with particular emphasis on those that are based on knowledge graphs. 
%
%Given a knowledge graph $\mathbf{KG}$, we define semantic relatedness as a function $\sigma: V\times V  \rightarrow \Re^+$, associating a positive score to every pair of nodes in the knowledge graph.  
%In this paper, we focus particularly on semantic relatedness in knowledge bases, with an emphasis on graph-based relatedness. 
%
% Too much hypothesizing  => Related work
%We hypothesize that good gist concepts should be strongly semantically related to most of the seed concepts.
%Several very recent measures have been researched for relatedness over knowledge graphs~\cite{Schuhmacher2014knowledge,Pirro2015Explaining,Hulpus2015pathbased}. 
%
%
We follow Hulpu{\c{s}} et al.\  \cite{Hulpus2015pathbased} who introduce the exclusivity-based measure, which we use as a node metric $\sigma^{(-1)}$. The authors found that it works particularly well on knowledge graphs of categories and article membership (which we use also) for modeling concept relatedness. It was shown to outperform simpler measures that only consider the length of the shortest path, or the length of top-k shortest paths, as well as the measure proposed in~\cite{Schuhmacher2014knowledge}.
%We therefore deem this measure reasonable for estimating graph-based entity relatedness. 

The exclusivity-based measure assigns a \emph{cost} for any edge $s\stackrel{r}{\rightarrow}t$ of type $r$ between source node $s$ and target node $t$. 
The cost function is the sum between the number of alternative edges of type $r$ starting from $s$ and the number of alternative edges of type $r$ ending in $t$, as shown in Formula~\ref{formula:cost}.

\begin{equation}
\scriptsize{}
\text{cost}(s\stackrel{r}{\rightarrow}t) = |\{s\stackrel{r}{\rightarrow}*\}| + |\{*\stackrel{r}{\rightarrow}t\}|-1,
\label{formula:cost}
\end{equation}

\noindent where $1$ is subtracted to count $s\stackrel{r}{\rightarrow}t$ only once. 

The more neighbors connected through the type of a particular edge, the less informative that edge is, and consequently the less evidence it bears towards the relatedness of its adjacent concepts.
By summing up the costs of all edges of a path $p$, one can compute the cost of that path, denoted $\text{cost}(p)$.
The higher the cost of a path, the lower its support for relatedness between the nodes at its ends. 
Thus, given two nodes, $s$ and $t$, their relatedness is computed as the inverse of the weighted sum of the costs of the top-$k$ shortest paths between them (ties are broken by cost function). 
Each path's contribution to the sum is weighted with a length based discounting factor $\alpha$: 
% \text{relatedness}(s,t)=
\begin{equation}
\scriptsize{}
\sigma(s,t)=\sum_{i=1}^k\alpha^{\text{length}(sp_i)}\times \frac{1}{\text{cost}(sp_i)}
\label{formula:relatedness}
\end{equation}  
\noindent where $sp_i$ denotes the $i$'th shortest path between $s$ and $t$.
$\alpha \in (0,1]$ is the length decay parameter and $k$ is a number of shortest paths to consider. 

%\simpletodo{Ioana: the relatedness measure takes 2 parameters: alpha, which in the experiments was set to 0.25 and k which was set to 3. I selected this setup as in the experiments on this relatedness this was the best setup. We must say this, by referring to my experiments saying - we choose these parameters as they were shown to perform best, and they are a good computational compromise, or we can experiment ourselves with different values of these parameters. In any case we must fence out this favourite reviewers' complaint that the choosing of parameters is not justified.  }





